A Robust Semantics-based Watermark for Large Language Model against Paraphrasing

Large language models (LLMs) have show great ability in various natural language tasks. However, there are concerns that LLMs are possible to be used improperly or even illegally. To prevent the malicious usage of LLMs, detecting LLM-generated text becomes crucial in the deployment of LLM applications. Watermarking is an effective strategy to detect the LLM-generated content by encoding a pre-defined secret watermark to facilitate the detection process. However, the majority of existing watermark methods leverage the simple hashes of precedent tokens to partition vocabulary. Such watermark can be easily eliminated by paraphrase and correspondingly the detection effectiveness will be greatly compromised. Thus, to enhance the robustness against paraphrase, we propose a semantics-based watermark framework SemaMark. It leverages the semantics as an alternative to simple hashes of tokens since the paraphrase will likely preserve the semantic meaning of the sentences. Comprehensive experiments are conducted to demonstrate the effectiveness and robustness of SemaMark under different paraphrases.

==> secs/intro_backup110315.tex <==
\section{Introduction}

Large language models (LLMs) have shown its great ability in various natural language processing (NLP) tasks like Question Answering (QA)~\cite{lu2022learn}, reasoning tasks~\cite{wei2022chain, creswell2022selection} and code development~\cite{xu2022systematic}. However, tremendous concerns have been raised that LLMs are possible to be used improperly and illegally. For example, fake news that are indistinguishable are easy to be fabricated~\citep{kreps2022all, zellers2019defending}, which, when disseminated, could instigate widespread panic. 
% In academic settings, there's potential for ghostwriters powered by LLMs to mislead educators~\citep{xie2023ai}. 
Similarly, in the commercial sphere, convincingly generated reviews can manipulate consumer perceptions, leading to unethical business competition~\citep{salminen2022creating}. 
Therefore, detecting AI-generated text has become crucial in the real-world applications of LLMs.

{Among diverse methods to detect AI-generated texts}, the watermark strategies have demonstrate outstanding precision~\citep{kirchenbauer2023watermark}. It is proposed to encode a secret watermark into the generated texts, such that one can tell whether a text is \yd{AI-generated} via detecting this watermark. One representative strategy~\cite{kirchenbauer2023watermark, yoo2023robust} is to encode the watermark based on the ``partition of vocabulary''. \yd{In particular}, 
% In detail, 
given a language model, these methods devise a mapping from precedent tokens to a particular partition of the vocabulary by a partition function for the consequent token. The partition function uses the hashes of the input as the seed of a random generator to split the vocabulary to a green list and a red list. During the text generation phase, the consequent token has an increased probability to be sampled from the green list. In this way, the watermark is encoded through the matching between the precedent tokens and the vocabulary partition for the consequent token. The detection is also facilitated by detecting this matching in generated contents. However, recent works~\cite{krishna2023paraphrasing, kaddour2023challenges} reveal that \textbf{this \yd{type of} watermark may be easily \yd{circumvented} by sentence paraphrasing}. 
Individuals seeking to \jr{improperly} utilize LLMs without being detected can paraphrase the generated contents, like altering the order and the choices of the words, \yd{while retaining} the general meaning of the text.
%%% comment by yd
% \jr{to achieve their malicious goals like faking news}. 
These paraphrases will change the seed of the partition function, i.e. the token hashes, and consequently disrupt the matching between the precedent tokens and the green list, \yd{which dramatically undermines the detection effectiveness.}
% . As a result, the detection effectiveness of the watermarks can be dramatically compromised.


In this paper, we propose to leverage the semantic meaning of precedent token sequences as the seed for partition function, instead of simple hashes of precedent tokens, since the core semantic meaning is expected to be maintained after paraphrasing. To achieve this goal, one key obstacle is how to capture the semantics when applying them for the partition function to watermark generated texts. It is a common practice to quantify the semantics via embeddings~\cite{reimers2019sentence, gao2021simcse, li2020sentence, giorgi2021declutr}. Embeddings indeed can represent consistent semantics after paraphrasing.  Since the embeddings are high-dimensional vectors in the continuous space, the embedding vectors could present some minor changes after paraphrasing. 
% \jt{I think we can have experiments to verify this claim}. 
\jr{These minor changes can lead to a substantial difference in the partition of vocabulary as the random generator in the partition function is sensitive to any change of the seed.}

% Intuitively, even if the content undergoes paraphrasing, the core semantic meaning remains consistent. Therefore, the watermark is likely to remain intact and detectable. Nevertheless, directly applying the semantics for the partition function faces tremendous challenges. 
% \jt{I think the logic below is not good. It is better to first discuss why the partiion function is sensitive to the input and it cannot understand the sematic . then you can explain even paragraph can maintain sematics, what will happen and what are the consequenec...}
% In detail, if we simply use the original embeddings for the partition of the green list of the next token, even slight paraphrase will make a difference to the vocabulary partition. Because the embeddings are in the continuous space and will \jt{what do you mean "have some alternation"} have some alternation under paraphrase even though the major semantics remain stable. This minor change can cause a great difference in the partition of vocabulary as the partition function is unaware of semantics and just uses the input as the seed of random generator to select green list.

To overcome this challenge, i.e., to make the quantified semantics invariant under paraphrase, we propose a new watermark method, SemaMark, which discretizes the continuous embedding space. Intuitively, the discretization can coarsen the representation of the embeddings which could tolerate the potential changes caused by paraphrase. By proper discretization, the paraphrased changes could exceed the same discrete section with a low probability and the quantified semantics will likely remain the same even after paraphrase. Therefore, the partition results will not change. However, directly converting the high-dimensional embedding space into discrete is intricate and challenging. For example, discretizing each dimension will lead to dense discrete values, i.e., the total number of discrete values is too large. 
% \jt{do not get what the following means?? Need to explain to me to let me understand}
Thus, one discrete value is not enough to accommodate the minor changes by paraphrase and the partitions changes are still unstable.
From another perspective, the change of only one discrete dimension can have a big impact on the partition function. 
% Second, the raw embeddings can be unevenly distributed in the whole space. If the semantics are unevenly concentrating in some discrete sections, the resulting discrete semantic values will be overly monotonous which raises the concern that the watermark might be cracked by counting token frequency~\cite{zhao2023provable}. 
% \jt{I think you can organize the following as: discuss the challenges of discretization and what are your solutions} 
To address this problem, SemaMark first uses a Multilayer Perception (MLP) to condense the continuous high-dimensional embeddings into normalized vectors in 2D space. The vectors are located on a unit circle named Normalized Embedding Ring (NE-Ring). Then the condensed NE-Ring is equally divided into various sections for distinct values, transforming the continuous space into discrete ``semantic values''. Based on the discretization, SemaMark further introduces two strategies to advance the watermark's concealment and improve the robustness under paraphrase. 
% \jt{I think it is a good practice to use short sentences instead of long sentences especially when we need to improve our English. Please rewrite the following }
\textit{First}, SemaMark leverages the uniformity~\cite{wang2020understanding} of Contrastive Learaning(CL)~\cite{chen2020simple} to strength the MLP and mitigate the situation that the semantics are unevenly concentrating on some discrete sections on NE-Ring. The unevenly distribution will cause the resulting discrete semantic values overly monotonous. It raises the concern that the watermark might be cracked by counting token frequency~\cite{zhao2023provable}. \textit{Second}, SemaMark utilizes an offset detection method to further increase the robustness at the boundary of different discrete sections whose semantic values are possibly vulnerable to paraphrase. Comprehensive experiments are provided to demonstrate its effectiveness and robustness under different paraphrase. 
% In this paper, we provide comprehensive experiments to demonstrate the performance of SemaMark in watermarking and its robustness under paraphrase.

% Experiments note

% Embeddings indeed can represent consistent semantics after paraphrasing.  Since the embeddings are high-dimensional vectors in the continuous space, the embedding vectors could present some minor changes after paraphrasing. 
% % \jt{I think we can have experiments to verify this claim}. 

% \jt{I think this could be the partition function is sensitive to the input??? do we verify? I think we should conduct some preliminary experiments to verify (1) changes on embeddings via paraphrasing (2) if the partition function is sensitive to the input changes??? } 

% \jt{as ablation study, we also need to verify if discretization can help??} 
